Variational Meta Reinforcement Learning for Social Robotics

With the increasing presence of robots in our every-day environments, improving their social skills is of utmost importance. Nonetheless, social robotics still faces many challenges. One bottleneck is that robotic behaviors need to be often adapted as social norms depend strongly on the environment. For example, a robot should navigate more carefully around patients in a hospital compared to workers in an office. In this work, we investigate meta-reinforcement learning (meta-RL) as a potential solution. Here, robot behaviors are learned via reinforcement learning where a reward function needs to be chosen so that the robot learns an appropriate behavior for a given environment. We propose to use a variational meta-RL procedure that quickly adapts the robots' behavior to new reward functions. As a result, given a new environment different reward functions can be quickly evaluated and an appropriate one selected. The procedure learns a vectorized representation for reward functions and a meta-policy that can be conditioned on such a representation. Given observations from a new reward function, the procedure identifies its representation and conditions the meta-policy to it. While investigating the procedures' capabilities, we realized that it suffers from posterior collapse where only a subset of the dimensions in the representation encode useful information resulting in a reduced performance. Our second contribution, a radial basis function (RBF) layer, partially mitigates this negative effect. The RBF layer lifts the representation to a higher dimensional space, which is more easily exploitable for the meta-policy. We demonstrate the interest of the RBF layer and the usage of meta-RL for social robotics on four robotic simulation tasks.

==> cover_letter.tex <==
\onecolumn

\begin{answereditor}

\qa{The article has serious criticism by the reviewers. Therefore you have to response point-by-point and revise the paper accordingly, The article must demonstrate novelty and technical contribution, with recent studies comparisons. Examine carefully, reviewers comments and answer separately one by one, label all change you would make on the revised revision, by colored fonts or underline so that each reviewer can trace carefully validate the change you may make.}
{Thank you for the suggestions. We have carefully revised the paper and provided answers to each of the Reviewers' comments individually. When there are changes in the manuscript associated with one of the questions, they are highlighted in the text in green with a label of the form ``Rn'', and in the cover letter, we refer to these changes indicating the change number and the page in the manuscript where it can be found.}

\qa{You also have to make sufficient checking for the paper organization and language by asking technical experts in English, like those in Springer. You may provide certificate that you have done such language checking.}
{We have requested the help of technical experts in English, and attach the certificate at the end of the cover letter.}


\qa{Also you need to look for recent studies and remove those that are more than 5 years, unless they are important. It is required that you look to further studies in high impact factor journals and limit to large extent those form conferences.}
{We have 53 references that are from after 2015 and 7 that are from before 2015. Among them, three are surveys on social robotics, and four are seminal papers (RBF, VAE, RL). We looked at the conference papers we refer to and replaced them with journal papers when an equivalent or an extension was found.}


\qa{In your submission you may provide graphical abstract as: using for example: \url{https://mindthegraph.com/blog/graphical-abstract-for-elsevier/?utm_campaign=article_of_the_future_novaid&utm_medium=email&utm_source=RD+Station}}
{We added a graphical abstract that shows the general working principle of the variational Meta-RL procedure in Figure~\ref{fig:teaser})}


\qa{Replace ArXiv papers(if any) (unless very related to the article research area) with related articles from high impact factor journals. These articles from arXiv are not reviewed and therefore you must look for reviewed journal related work from \url{www.sciencedirect.com}.}
{
We checked for all our arxiv references if the paper was officially published and adapted the references for these papers. Only a few references to arxiv manuscripts remain, as they were not published, no equivalent was found, and they are key for understanding our work. 
}

 
\end{answereditor}

\begin{answerreviewer}

% {This paper investigates the use and limitations of variational meta-RL for social robotics. An RBF network is added to the meta-RL to mitigate the posterior collapse. Overall, the paper is well-written. My comments can be found below:}
% \newline
% \newline

\qa{In the part of the introduction (section 1), it is not clear to me what is the novelty of the first contribution. It seems that this paper just applies meta-RL to different tasks. Has the meta-RL been applied to the same research topic? These points should be discussed in detail.}
{Thanks for this question. To our knowledge, the use of meta-RL for social robotics has been only scarcely investigated. More precisely, previous work only explored the use of on-policy meta-RL, which requires lots of interaction with the environment (environment steps) to obtain satisfactory performances. We discuss this point in~\refcm{meta-rl-social-bots}.}

\qa{This paper suggests an MDP and a single-agent method. However, there may exist some situations that require cooperation between agents. Is it possible to extend the proposed framework into a multi-agent setup? Please discuss it.}
{Thanks for the suggestion. We discuss the possibility of extending the proposed framework into a multi-agent setup in ~\refcm{marl}}

\qa{Can the safety of the proposed meta-RL method be ensured during the test or even training processes, i.e., without any constraint/limit violations?}
{Safety is indeed crucial in social robotics. We examine the limitation of meta-RL on ensuring safety constraints in ~\refcm{safety} }

\qa{Is it realistic to assume that the agent can always get the complete observation information? What if the observation information is incomplete? How does it influence training performance?}
{Thanks for the question. We talk about how meta-RL adapts to an environment with incomplete information in ~\refcm{pomdp}}

\qa{Minor comments: (1) In Fig.4, it seems that the caption has a typo. The sub-figure in the left hand is 'linear gaze control'.} 
{Corrected, see Fig~\ref{fig:gaze_results}.}

\qa{Minor comments: (2) Please discuss why the PEARL method will suffer from posterior collapse. Is it enough to only use RBF to mitigate this issue?}
{Posterior collapse is a recurrent issue in VAE-based deep learning architectures. Roughly speaking, posterior collapse occurs when the encoder does not need to use all the dimensions of the latent variable to represent the variability of the observed data distribution. However, this also depends on the training dynamics. In practice, once one of the dimensions of the latent space is collapsed, it cannot be used anymore for training, and regular optimization schemes cannot exploit this latent variable dimension anymore. The RBF helps to mitigate this issue, as reported in our extensive experimental study.}

\qa{Minor comments: (3) It may be better to avoid the use of lumped references. A table could be very useful to show the detailed comparison between existing papers in this research area.}
{We restructured our "Related work" section \refcm{relatedwork} to focus on more relevant aspects and to avoid the use of lumped references.
We introduced more survey papers about our relevant topics: Social Robotics, Adaptive Social Robotics, RL in Social Robotics, and Meta-RL.
Our paper explores for the first time the use of off-policy meta-RL for social robotics. 
As such, the most relevant methods are other meta-RL methods. 
Since there exists a recent review on meta-RL~\cite{beck2023survey}, we believe providing such a comprehensive taxonomy of the methods is out of the scope of the current paper. 
However, on top of the detailed description of PEARL, and PEARL-RBF, we provide a brief description of two on-policy meta-RL methods used in our experimental benchmark, see~\refcm{baselines}.
% is a method paper that cites only the most relevant related work.
% It is not a comprehensive survey that tries to give a taxonomy of the research field.
% Thus, we believe that a table is not necessary and only increases the length of the paper without giving much more information.
}

\end{answerreviewer}

\begin{answerreviewer}

% This manuscript APIN-D-22-07563 investigates meta-reinforcement learning (meta-RL) as a potential solution. Here, robot behaviors are learned via reinforcement learning where a reward function needs to be chosen so that the robot learns an appropriate behavior for a given environment. The authors propose to use a variational meta-RL procedure that quickly adapts the robots' behavior to new reward functions. As a result, given a new environment different reward functions can be quickly evaluated and an appropriate one selected. The procedure learns a vectorized representation for reward functions and a meta-policy that can be conditioned on such a representation. Given observations from a new reward function, the procedure identifies its representation and conditions the meta-policy to it. While investigating the procedures' capabilities, the authors realized that it suffers from posterior collapse where only a subset of the dimensions in the representation encode useful information resulting in a reduced performance. The second contribution, a radial basis function (RBF) layer, partially mitigates this negative effect. It was a pleasure reviewing this work and I can recommend it for publication in Applied Intelligence after a major revision. I respectfully refer the authors to my comments below.
% \newline
% \newline


\qa{The English needs to be revised throughout. The authors should pay attention to the spelling and grammar throughout this work. I would only respectfully recommend that the authors perform this revision or seek the help of someone who can aid the authors.}
{Thanks for the suggestion. We had our manuscript checked by an expert, the certificate is attached after the cover letter.}

\qa{(References) Please adjust the style of all the references to meet the Applied Intelligence requirement.}
{We used the style that is defined by the Springer Latex template which should be used for submissions (\url{https://www.springer.com/journal/10489/submission-guidelines}). If a different style needs to be used, we will be very happy to use it, but we could not find any information other than the referenced webpage.}
% We do not have access to the final latex style file of Applied Intelligence.
% We will adapt the references when we receive it to prepare a camera-ready version. \xavi{Sure, but I have corrected also many references in the bib file. They were set as ``article'' but they were ``inproceedings''.}

\qa{(Page 8) The original figures 2-3 are not clear. Please redraw this figure clearly. Add some word in this figure, and indicate the imaging modules.}
{Thanks for the feedback. These Figures became now Fig~\ref{fig:graph} and~\ref{fig:gaze_env} respectively. The new Figure~\ref{fig:graph} has been redesigned to put forward how the RBF layer is working, and how it is integrated within the PEARL environment. We came up with a graphical description of how the output RBF representation is obtained, and we sincerely hope it is more clear now. Regarding Figure~\ref{fig:gaze_env}, we have drawn the scene outside the field of view in grayscale, and we add a few annotations to the image to make it easier to understand.}

\qa{(Section 1 Introduction) The reviewer hopes the introduction section in this paper can introduce more studies in recent years. The reviewer suggests authors don't list a lot of related tasks directly. It is better to select some representative and related literature or models to introduce with certain logic. For example, the latter model is an improvement on one aspect of the former model.}
{We significantly improved the discussion according to the proposal of the reviewer. See~\refcm{relatedwork} and Q7 of R1.
}

\qa{Experimental pictures or tables should be described and the results should be analyzed in the picture description so that readers can clearly know the meaning without looking at the body.}
{We did our best to adapt the captions of Figures~\ref{fig:gaze_results}, \ref{fig:social_nav_results}, and~\ref{fig:racer_results} to accommodate the suggestion of the reviewer. We sought a trade-off between the caption being not too long yet self-content.}

\qa{(Page 2, In Section 1 Introduction) The original sentence is revised as "models and the representation power of deep neural networks [*] …."(NGDNet: Nonuniform Gaussian-label distribution learning for infrared head pose estimation and on-task behavior understanding in the classroom. Neurocomputing 2021; Facial expression recognition method with multi-label distribution learning for non-verbal behavior understanding in the classroom. 2021)}
{Thank you for your suggestion. We have added the reference to NGDNet, and also to a recent review on dynamical variational autoencoders to broaden the scope beyond the education-oriented contribution on infrared head-pose estimation, see~\refcm{extra-refs-1}.}

\qa{(Tables 1 and Page 15) All the values in this table should be with the same data accuracy. The number of data after the decimal point is the same. Please check other Tables and section "Influence on the learned input task representation z".}
{We are not completely sure that we understand the suggestion correctly.
The table is about the performance, measured as the return of each algorithm.
The values in the text body are about the spread of representations in their respective space. The numbers in the body text provide now the same number of decimal points. We hope this is what you meant.
}

\qa{The original sentence is suggested to revise as "the deployment of interactive robots in different environments, such as malls $<$arhpe: asymmetric relation-aware representation learning for head pose estimation in industrial human-computer interaction $>$, offices $<$ ehpe: skeleton cues-based gaussian coordinate encoding for efficient human pose estimation $>$, or hospitals $<$mfdnet: collaborative poses perception and matrix fisher distribution for head pose estimation$>$ ."}
{Thank you for the suggestions. We added ARHPE as an example of social robotics deployment in industrial applications. We also added two other references discussing the deployment of social robots in healthcare and educational facilities. We believe that the two other references suggested by the reviewer, while valuable contributions to head-pose estimation, are too focused on pose estimation to be in the first sentence of a paper on meta-RL for social robotics, see~\refcm{deployment}.}

\qa{The authors are suggested to add some experiments with the methods proposed in other literature, then compare these results with yours, rather than just comparing the methods proposed by yourself on different models.}
{Thank you for the suggestion. We added two sets of experiments with state-of-the-art baselines proposed in other literature and then compared the results they obtained with ours ~\refcm{baselines}, ~\refcm{baselines-gazecontrol}, ~\refcm{baselines-racer}, ~\refcm{baselines-crowd}. Our method generally outperforms these baselines which are less sample efficient than ours.}

\qa{Discuss the pros and cons of the proposed models.}
{We provide a discussion about the pros and cons of on-policy meta-RL models and off-policy meta-RL models in~\refcm{discussion-models}. We argue that our method is more suited for robotics and especially social robotics as it is more sample efficient than concurrent methods in the literature.}

\end{answerreviewer}

% \vspace{1.5cm}
% {\LARGE\color{red} THE FOLLOWING HAS TO BE REMOVED}\\

% E-mail to the Journal \& EiC\\

% E-mail addresses:\\
% Hariini Chandrasekaran: (hariini.chandrasekaran@springernature.com)\\
% Hamido Fujita: (hfujita@i-somet.org)\vspace{1cm}\\

% Dear Prof. Hamido Fujita and Hariini Chandrasekaran,

% We are the authors of the Applied Intelligence submission APIN-D-22-07563. We write you because we would like to send a confidential e-mail to the Associated Editor handling our submission. However, we did not find any way of contacting the AE directly, thus we send you this communication.

% We have worked toward modifying the manuscript according to the valuable remarks of the reviewers. We are happy to broaden the discussion to the topics suggested by the reviewers, and to extend the experimental study. We believe that their suggestions were very useful. 

% Among the comments of Reviewer 2, we find two sentence reformulations that suggest to add five new citations (altogether). After taking a look to these references [1-5], we observe that all of them satisfy two criteria: (i) they authored by Tingting Liu, or by Zhiqiang Zhang, or by both, (ii) in our humble opinion they are not always the best references to add in the respective sentences. Thus we replaced some of the suggested references for others.

% We provided all details in the cover letter of our article (and just below), and with this e-mail we would like to make sure that the Associate Editor is aware of the rationale of our choice. We are happy to engage in further discussion should it be needed. 

% In details, we have added reference [1] to our manuscript, and replace the suggestion [2] by a recent review of ours on dynamical variational autoencoders [A]. This broadens the discussion toward a more methodological grounding beyond the classroom-oriented application of [1,2].

% Regarding the second set of references suggested by the reviewer [3,4,5], we believe that while [3] has some application to industrial robotics, [4,5] are focused exclusively on head pose estimation (and are very valuable contributions in this regard), and are therefore too narrow to be cited in the first sentence of a paper on reinforcement learning for social robotics. In order to support our first statement, we added two other references discussing the deployment of social robotics in healthcare [B] and education facilities [C].

% References suggested by Reviewer 2
% [1] Liu, Tingting, Jixin Wang, Bing Yang, and Xuan Wang. "NGDNet: Nonuniform Gaussian-label distribution learning for infrared head pose estimation and on-task behavior understanding in the classroom." Neurocomputing 436 (2021): 210-220.
% [2] Liu, Tingting, Jixin Wang, Bing Yang, and Xuan Wang. "Facial expression recognition method with multi-label distribution learning for non-verbal behavior understanding in the classroom." Infrared Physics \& Technology 112 (2021): 103594.
% [3] Liu, Hai, Liu, Tingting, Zhang, Zhaoli, Sangaiah, Arun Kumar, Yang, Bing, and LiLiu, Youfu, "ARHPE: Asymmetric Relation-Aware Representation Learning for Head Pose Estimation in Industrial Human–Computer Interaction." IEEE Trans. Ind. Inform 18 (2022): 7107-7117.
% [4] Liu, Hai, Tingting Liu, Yu Chen, Zhaoli Zhang, and You-Fu Li. "EHPE: skeleton cues-based gaussian coordinate encoding for efficient human pose estimation." IEEE Transactions on Multimedia (2022).
% [5] Liu, Hai, Shuai Fang, Zhaoli Zhang, Duantengchuan Li, Ke Lin, and Jiazhang Wang. "MFDNet: Collaborative poses perception and matrix Fisher distribution for head pose estimation." IEEE Transactions on Multimedia 24 (2021): 2449-2460.

% Added references
% [A] Girin, L., Leglaive, S., Bie, X., Diard, J., Hueber, T. and Alameda-Pineda, X., 2021. Dynamical Variational Autoencoders: A Comprehensive Review. Foundations and Trends in Machine Learning, 15(1-2), pp.1-175.
% [B] Kubota, A., Peterson, E.I., Rajendren, V., Kress-Gazit, H. and Riek, L.D., 2020, March. Jessie: Synthesizing social robot behaviors for personalized neurorehabilitation and beyond. In Proceedings of the 2020 ACM/IEEE international conference on human-robot interaction (pp. 121-130).
% [C] Davison, D.P., Wijnen, F.M., Charisi, V., van der Meij, J., Evers, V. and Reidsma, D., 2020, March. Working with a social robot in school: a long-term real-world unsupervised deployment. In Proceedings of the 2020 ACM/IEEE international conference on human-robot interaction (pp. 63-72).


% Best regards,
% Xavier Alameda-Pineda, on behalf of the authors of APIN-D-22-07563

\clearpage
\includepdf{Attestation.pdf}
\twocolumn
